NoWag: A Unified Framework for Shape Preserving Compression of Large Language Models

Large language models (LLMs) exhibit remarkable performance across various natural language processing tasks but suffer from immense computational and memory demands, limiting their deployment in resource-constrained environments. To address this challenge, we propose NoWag (Normalized Weight and Activation Guided Compression), a unified framework for one-shot shape preserving compression algorithms. We apply NoWag to compress Llama-2 (7B, 13B, 70B) and Llama-3 (8B, 70B) models using two popular shape-preserving techniques: vector quantization (NoWag-VQ) and unstructured/semi-structured pruning (NoWag-P). Our results show that NoWag-VQ significantly outperforms state-of-the-art one-shot vector quantization methods, while NoWag-P performs competitively against leading pruning techniques. These findings highlight underlying commonalities between these compression paradigms and suggest promising directions for future research. Our code is available at https://github.com/LawrenceRLiu/NoWag

==> Algorithms/normalization.tex <==
\begin{algorithm}[H]
\fontsize{7pt}{8pt}\selectfont\
\caption{\method Normalization}\label{alg:normalization}
\begin{algorithmic}[0]
\REQUIRE Weight matrix $W \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$
\ENSURE Normalized weight matrix $\bar{W}$, normalization vectors $r^{(1)}$, $r^{(2)}$
\STATE Compute column norms: $r^{(1)}_j = \sqrt{\sum_{i=1}^{d_{\text{out}}} W_{ij}^2}$ for $j \in [1, d_{\text{in}}]$
\STATE Normalize columns: $W'_{ij} = \frac{W_{ij}}{r^{(1)}_j + \varepsilon} \forall i,j$
\STATE Compute row norms: $r^{(2)}_i = \sqrt{\sum_{j=1}^{d_{\text{in}}} {W'}_{ij}^2}$ for $i \in [1, d_{\text{out}}]$
\STATE Normalize rows: $\bar{W}_{ij} = \frac{W'_{ij}}{r^{(2)}_i + \varepsilon} \forall i,j$

\RETURN $\bar{W}$, $r^{(1)}$, $r^{(2)}$
\end{algorithmic}
\end{algorithm}


==> Algorithms/padding.tex <==

\begin{algorithm}
\caption{VQ Padding}\label{alg:padding}
\begin{algorithmic}[1]
\REQUIRE Normalized weight matrix $\bar{W} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$, input dimension $d_{\text{in}}$, subvector dimension $d$
\ENSURE Padded weight matrix $\bar{W}_{\text{padded}}$, padded input dimension $d_{\text{in}}^{\text{padded}}$

\IF{$d_{\text{in}} \bmod d \neq 0$}
    \STATE $\text{pad\_size} \leftarrow d - (d_{\text{in}} \bmod d)$ 
    \STATE $\text{pad\_value} \leftarrow \text{mean}(\bar{W})$
    \STATE Pad $\bar{W}$ with $\text{pad\_value}$ to shape $(d_{\text{out}}, d_{\text{in}} + \text{pad\_size})$
    \STATE $d_{\text{in}}^{\text{padded}} \leftarrow d_{\text{in}} + \text{pad\_size}$
\ELSE
    \STATE $\bar{W}_{\text{padded}} \leftarrow \bar{W}$ 
    \STATE $d_{\text{in}}^{\text{padded}} \leftarrow d_{\text{in}}$
\ENDIF

\RETURN $\bar{W}_{\text{padded}}$, $d_{\text{in}}^{\text{padded}}$
\end{algorithmic}
\end{algorithm}

==> Algorithms/pruning.tex <==
\begin{algorithm}
\caption{\method Pruning (\methodP) TODO: REMOVE GROUPING}\label{alg:pruning}
\begin{algorithmic}[1]
\REQUIRE Weight matrix $W \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$, activation samples $X \in \mathbb{R}^{m \times d_{\text{in}}}$, target sparsity $s$, sparsity pattern $P \in \{\text{unstructured}, \text{N:M}\}$
\ENSURE Pruned weight matrix $\hat{W}$

\STATE $(r^{(1)}, r^{(2)}, \bar{W}) \leftarrow \texttt{\method\_Normalization}(W)$ \COMMENT{Apply normalization}
\STATE $S_{ij} \leftarrow \bar{W}_{ij}^2 \cdot \|X_j\|_2^2, \forall i \in [1,d_{\text{out}}], \forall j \in [1,d_{\text{in}}]$ \COMMENT{Importance scores}

\IF{Pattern is \text{unstructured}}
    \STATE $\tau \leftarrow $ \COMMENT{$s$-th percentile of all elements in $S$}
    \STATE $M \leftarrow \mathbf{1}_{S > \tau}$ \COMMENT{Binary mask where $M_{ij} = 1$ if $S_{ij} > \tau$, else 0}
\ELSIF{Pattern is \text{N:M}}
    \FOR{each row $i \in [1,d_{\text{out}}]$}
        \FOR{$g = 0$ to $\lfloor d_{\text{in}}/M \rfloor - 1$}
            \STATE $I_g \leftarrow \{gM + 1, gM + 2, \ldots, gM + M\}$ \COMMENT{Indices of group $g$}
            \STATE $T_g \leftarrow \text{top-N}(\{S_{ij} : j \in I_g\})$ \COMMENT{Indices of top N scores}
            \STATE $M_{ij} \leftarrow \begin{cases} 1 & \text{if } j \in T_g \\ 0 & \text{otherwise} \end{cases}, \forall j \in I_g$ \COMMENT{Set mask}
        \ENDFOR
    \ENDFOR
\ENDIF

\STATE $\hat{W} \leftarrow W \odot M$ \COMMENT{Element-wise multiplication}

\RETURN $\hat{W}$
\end{algorithmic}
\end{algorithm}

==> Algorithms/vq.tex <==

 % or {\footnotesize for even smaller
\begin{algorithm}\fontsize{7pt}{8pt}\selectfont
\caption{\methodVQ}\label{alg:vq} 
\begin{algorithmic}[0] 
\REQUIRE Weight matrix $W \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$, activation samples $X \in \mathbb{R}^{m \times d_{\text{in}}}$, subvector dimension $d$, bits per value $n_{\text{bits}}$, number of iterations $n_{\text{iter}}$ 
\ENSURE Quantized weight matrix $\hat{W} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$, codebook $C$, assignments $A$ 
\STATE $(r^{(1)}, r^{(2)}, \bar{W}) \leftarrow \texttt{\method Normalization}(W)$ \COMMENT{See Algorithm~\ref{alg:normalization}}
\STATE $(\bar{W}_{\text{padded}}, d_{\text{in, padded}}) \leftarrow \texttt{VQPadding}(\bar{W}, d_{\text{in}}, d)$ \COMMENT{See Algorithm~\ref{alg:padding}}
\STATE $H_j \leftarrow \|X_j\|_2^2, \forall j \in [1, d_{\text{in}}]$ \COMMENT{Diagonal of sample hessian} 
\IF{$d_{\text{in}} \neq d_{\text{in, padded}}$} 
\STATE Pad $H$ with zeros to length $d_{\text{in, padded}}$ 
\ENDIF 
\STATE Reshape $\bar{W}_{\text{padded}}$ into subvectors: $\bar{W}_{\text{sub}} \in \mathbb{R}^{N \times d}$ where $N = \frac{d_{\text{out}} \times d_{\text{in, padded}}}{d}$ 
\STATE Reshape $H$ into subvector weights: $H_{\text{sub}} \in \mathbb{R}^{N \times d}$ 
\STATE $n_{\text{centroids}} \leftarrow 2^{n_{\text{bits}} \cdot d}$ 
\STATE $(C, A) \leftarrow \texttt{Weighted\_KMeans}(\bar{W}_{\text{sub}}, H_{\text{sub}}, n_{\text{centroids}}, n_{\text{iter}})$ \COMMENT{See Algorithm~\ref{alg:wkmeans}}
\STATE $\hat{W}_{\text{sub}} \leftarrow$ Map each subvector to its assigned centroid using $A$ 
\STATE Reshape $\hat{W}_{\text{sub}}$ back to matrix form and remove padding to get $\hat{W} \in \mathbb{R}^{d_{\text{out}} \times d_{\text{in}}}$ \COMMENT{Reverses padding from Algorithm~\ref{alg:padding}}
\RETURN $\hat{W}$, $C$, $A$ 
\end{algorithmic} 
\end{algorithm}




==> Algorithms/wkmeans.tex <==

\begin{algorithm}
\caption{Weighted K-Means with K-Means++ Initialization}\label{alg:wkmeans}
\begin{algorithmic}[1]
\REQUIRE Subvectors $\bar{W}_{\text{sub}} \in \mathbb{R}^{N \times d}$, importance weights $H_{\text{sub}} \in \mathbb{R}^{N \times d}$, number of centroids $n_{\text{centroids}}$, number of iterations $n_{\text{iter}}$
\ENSURE Codebook $C \in \mathbb{R}^{n_{\text{centroids}} \times d}$, assignments $A \in \mathbb{R}^{N}$

\STATE \textbf{Initialize codebook} $C \in \mathbb{R}^{n_{\text{centroids}} \times d}$:
\STATE Select random indices $I = \{i_1, i_2, \ldots, i_{n_{\text{centroids}}}\}$ from $[1, N]$ without replacement
\STATE $C_l \leftarrow \bar{W}_{\text{sub},i_l}, \forall l \in [1,n_{\text{centroids}}]$

\FOR{$t = 1$ to $n_{\text{iter}}$}
    \STATE \textbf{Assignment step:} 
    \FOR{each subvector $i \in [1,N]$}
        \STATE $D_{i,l} \leftarrow \sum_{j=1}^{d} H_{\text{sub},i,j} \cdot (\bar{W}_{\text{sub},i,j} - C_{l,j})^2, \forall l \in [1,n_{\text{centroids}}]$
        \STATE $A_i \leftarrow \arg\min_{l} D_{i,l}$ 
    \ENDFOR
    
    \STATE \textbf{Update step:}
    \FOR{each centroid $l \in [1,n_{\text{centroids}}]$}
        \STATE $S_l \leftarrow \{i : A_i = l\}$ 
        \IF{$S_l \neq \emptyset$}
            \FOR{dimension $j \in [1,d]$}
                \STATE $C_{l,j} \leftarrow \frac{\sum_{i \in S_l} H_{\text{sub},i,j} \cdot \bar{W}_{\text{sub},i,j}}{\sum_{i \in S_l} H_{\text{sub},i,j}}$ \COMMENT{Weighted average}
            \ENDFOR
        \ENDIF
    \ENDFOR
    
    \STATE \textbf{Convergence check for no change in assignments TODO WRITE LINE BETTER}
\ENDFOR

\RETURN $C$, $A$
\end{algorithmic}
\end{algorithm}

==> Figures/corr.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/correlation_between_wanda_and_our_grouping.png}
    \caption{Histogram of the per Layer relative agreement in pruning location between \methodP and Wanda without (blue) and with output group pruning (orange). Calibration dataset for all was 128 samples of RedPajamas. Our Normalization behaves similarly to output group based pruning.}
    \label{fig:weight_distribution}
\end{figure}

==> Figures/sparse_mask.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Figs/layer_0-self_attn.q_proj_unstructured.png}
    \caption{Plot of the masks of pruned and unprunded elements with Wanda without grouping (left), with grouping (center) and with \methodP (right), for 50$\%$ unstructured pruning, \red{Black} is the preserved elements, white is the pruned.}
    \label{fig:weight_distribution}
\end{figure}

==> Figures/weights.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{"Figs/layer_0-self_attn.q_proj_weights.png"}
    \caption{Left, plot of the original weight matrix without normalization, right the plot of the normalized weight, columns and rows with large norms have been broken up}
    \label{fig:weight_plota}
\end{figure}

==> Sections/Appendices/Normalization.tex <==
%figs needed
%distribution fig

%
\section{Effect of Normalization on Weights}
\label{app:Normalization}
% \red{
% TODOs:
% \begin{itemize}
%     \item add colorbar to Fig 2
%     \item add 
% \end{itemize}
% }
Below are two plots illustrating the effects of normalization has on the weights. For both plots, we used the weights of the Q projection of the first layer of the Llama 2 7B parameter model. In figure \ref{fig:weight_plot}, we plot out the weights before and after normalization, and in figure \ref{fig:weight_distribution} we plot out the distribution of the consecutive groups of 6 elements that we quantized together with \methodVQ.
\input{Figs/weight_dist}
\input{Figs/weights}
\subsection{Effect of Normalization On Sparsity}
Below, we examine the effects of the normalization on the resulting locations of the pruned weights. Empirically, as shown in in figures \ref{fig:weight_distributiona} and \ref{fig:weight_plota}, normalization appears to have a similar impact as output group based pruning.
\input{Figs/sparse_mask}
\input{Figs/corr}


==> Sections/ToDOs.tex <==
%my own list of things
\red{
\begin{itemize}
    \item Finetune Llama 2 7B and Llama 3 8B.
    \item Finish Quantizing Llama 2 70B (done), and Llama 3 70B.
    \item Discuss if we need 3 bit quantization
    \item Update plots of weight distribution post normalization to main body
    \item Move Wanda Correlations to main body (maybe redo)?
    \item Redo Zeroshot on newest LM-Harness
    \item Talk with CMU about Wanda reproducibility (talking rn)
    \item Run QuIP\# so we can get Zero-shot accuracies. (Not Necessary imo)
    \item Trellis Quantization
    \item One Shot or Zero Shot?
\end{itemize}
}
% - Llama 2 70B (running) and Llama 3 70B 
% - get finetuning done
% - run ablation for different amounts of calibration data vs quip sharp, and maybe wanda
% - get wanda and sparsegpt to run at c4
% - maybe low rank compression


==> Tabels/sensitivity_T.tex <==
\begin{table}[H]
\centering
\small

\begin{tabular}{l | c c c | c c c |}
\toprule
 & \multicolumn{3}{c|}{Wikitext2 PPL $(\downarrow)$} & \multicolumn{3}{c|}{C4 PPL $(\downarrow)$}\\

 & (2-7B) & (2-13B) & (3-8B) & (2-7B) & (2-13B) & (3-8B) \\
 \hline
QuIP\# & 8.23 & 6.06 & 13.80 & 10.80 & 8.07 & 15.60 \\
\gr \methodVQ $T=1$ & \textbf{7.32} & 6.20 & \textbf{12.44} & \textbf{9.58} & 8.36 & \textbf{13.96} \\
\gr \methodVQ $T=10$ & 7.04 & \textbf{6.00} & 11.08 & 9.19 & \textbf{8.03} & 12.35 \\
\gr \methodVQ $T=40$ & 7.10 & 5.99 & 10.86 & 9.15 & 7.98 & 12.07 \\
\gr \methodVQ $T=100$ & 7.07 & 5.93 & 10.68 & 9.12 & 7.94 & 11.92 \\
\bottomrule
\end{tabular}

\caption{Ablation for $T=1,10,40$ against the default $T=100$ for \methodVQ for Llama-2-7b/13b and Llama-3 8B. We listed the Wikitext2 and C4 perplexities below, \textbf{bolding} the smallest for which NoWag outperforms QuIP\#. For Llama-2 7b and Llama-3 8B NoWag with only one iteration of K-means was able to outperform QuIP\#, for Llama-2 13B, after 10 iterations, NoWag-VQ was able to outperform QuIP\#. We also note that the performance of the model continues to increase as we increase the number of iterations.}
\label{tab:ablation_T}
\end{table}
